Beyond Single Concept Vector: Modeling Concept Subspace in LLMs with Gaussian Distribution

Probing learned concepts in large language models (LLMs) is crucial for understanding how semantic knowledge is encoded internally. Training linear classifiers on probing tasks is a principle approach to denote the vector of a certain concept in the representation space. However, the single vector identified for a concept varies with both data and training, making it less robust and weakening its effectiveness in real-world applications. To address this challenge, we propose an approach to approximate the subspace representing a specific concept. Built on linear probing classifiers, we extend the concept vectors into Gaussian Concept Subspace (GCS). We demonstrate GCS's effectiveness through measuring its faithfulness and plausibility across multiple LLMs with different sizes and architectures. Additionally, we use representation intervention tasks to showcase its efficacy in real-world applications such as emotion steering. Experimental results indicate that GCS concept vectors have the potential to balance steering performance and maintaining the fluency in natural language generation tasks.

==> prompts.tex <==
\begin{longtable}{>{\centering\arraybackslash}m{2.2cm}|>{\centering\arraybackslash}m{2.7cm}|>{\centering\arraybackslash}m{1cm}|>{\raggedright\arraybackslash}p{7cm}}
\caption{Complex table structure with wrapped text in the last column}\label{tab:complex}\\

\hline\hline
High-level concept & Low-level concept & Pos/Neg & Prompts\\\hline\hline
\endfirsthead

\multicolumn{4}{c}{Table \thetable{} continued from previous page} \\
\hline\hline
High-level concept & Low-level concept & Pos/Neg & Prompts\\\hline\hline
\endhead

\hline\multicolumn{4}{r}{\small Continued on next page}
\endfoot

\hline\hline
\endlastfoot

\multirow{8}{*}[-1em]{\centering Sports Event} & \multirow{2}{*}[-0.5em]{Cycling competition} & P \\ \cline{3-4}
&& N \\ \cline{2-4}
& \multirow{2}{*}[-0.5em]{Football match} & P \\ \cline{3-4}
&& N \\ \cline{2-4}
& \multirow{2}{*}[-0.5em]{Tennis tournament} & P \\ \cline{3-4}
&& N \\ \cline{2-4}
& \multirow{2}{*}[-0.5em]{Motor race} & P \\ \cline{3-4}
&& N \\ \hline

\multirow{8}{*}[-1em]{\centering Populated Place} & \multirow{2}{*}[-0.5em]{Town} & P \\ \cline{3-4}
&& N \\ \cline{2-4}
& \multirow{2}{*}[-0.5em]{Island} & P \\ \cline{3-4}
&& N \\ \cline{2-4}
& \multirow{2}{*}[-0.5em]{City district} & P \\ \cline{3-4}
&& N \\ \cline{2-4}
& \multirow{2}{*}[-0.5em]{Village} & P \\ \cline{3-4}
&& N \\ \hline

\multirow{8}{*}[-1em]{\centering Movie} & \multirow{2}{*}[-0.5em]{Horror} & P & Generate a horror movie description that focuses on supernatural elements, eerie atmospheres, and terrifying creatures. The plot should involve a haunted house, a cursed object, or a series of inexplicable events. The protagonist should be a brave or desperate individual who must confront the supernatural forces at play. Make sure the tone is dark and suspenseful, with a focus on fear and paranoia. The text should be at most 30 words. Please include 'horror movie' in these texts and generate 100 samples. \\ \cline{3-4}
&& N \\ \cline{2-4}
& \multirow{2}{*}[-0.5em]{Action} & P & Generate an exciting movie description that highlights intense action sequences, fast-paced chases, physical confrontations, and daring stunts. The plot should involve high stakes, such as saving the world, defeating a villain, or completing a dangerous mission. The protagonist should be a courageous hero facing impossible odds. Make sure the tone is intense and thrilling. The text should be at most 30 words. Please include 'action movie' in these texts and generate 100 samples. \\ \cline{3-4}
&& N \\ \cline{2-4}
& \multirow{2}{*}[-0.5em]{Comedy} & P & Write a lighthearted and humorous movie description filled with funny situations, witty dialogue, and comical misunderstandings. The story should involve likable characters in everyday or ridiculous scenarios, and the tone should be playful and uplifting. The protagonist could be dealing with awkward social situations, family dynamics, or a series of humorous accidents. The text should be at most 30 words. Please include 'comedy movie' in these texts and generate 100 samples. \\  \cline{3-4}
&& N \\ \cline{2-4}
& \multirow{2}{*}[-0.5em]{Sci-Fi} & P \\ \cline{3-4}
&& N \\ \hline

\multirow{8}{*}[-1em]{\centering Animal} & \multirow{2}{*}[-0.5em]{Bird} & P \\ \cline{3-4}
&& N \\ \cline{2-4}
& \multirow{2}{*}[-0.5em]{Fish} & P \\ \cline{3-4}
&& N \\ \cline{2-4}
& \multirow{2}{*}[-0.5em]{Insect} & P \\ \cline{3-4}
&& N \\ \cline{2-4}
& \multirow{2}{*}[-0.5em]{Cat} & P \\ \cline{3-4}
&& N \\
\end{longtable}

